Pruning, Pushdown Exception-Flow Analysis

Statically reasoning in the presence of exceptions and about the effects of exceptions is challenging: exception-flows are mutually determined by traditional control-flow and points-to analyses. We tackle the challenge of analyzing exception-flows from two angles. First, from the angle of pruning control-flows (both normal and exceptional), we derive a pushdown framework for an object-oriented language with full-featured exceptions. Unlike traditional analyses, it allows precise matching of throwers to catchers. Second, from the angle of pruning points-to information, we generalize abstract garbage collection to object-oriented programs and enhance it with liveness analysis. We then seamlessly weave the techniques into enhanced reachability computation, yielding highly precise exception-flow analysis, without becoming intractable, even for large applications. We evaluate our pruned, pushdown exception-flow analysis, comparing it with an established analysis on large scale standard Java benchmarks. The results show that our analysis significantly improves analysis precision over traditional analysis within a reasonable analysis time.

==> benchmarks-table-precision.tex <==
%
%% % % current results, I will consider to add time. too.
%\begin{table}
%\centering
%{\footnotesize
%    \begin{tabular}{ c| c| c | c | c | c | c | c | c| c| }
%    \textbf{Precision}  &  \textbf{antlr} & \textbf{bloat} & \textbf{chart} & \textbf{fop} & \textbf{hsqldb} & \textbf{luindex} & \textbf{lusearch}   & \textbf{pmd}  & \textbf{xalan}  \\ \hline 
%     \multirow{2}{*}{} &  pdxfa+1obj  & 13.3x & 9.8x & 25.9x   &  12.5x & 16.3x  & 7.6x & 6.7x & 18.4x 
%  \\
%       & pdxfa + eagc &   11.7x  &  5.9x &14.9x & 10.9x & 5.4x  & 2.7& 5.7x & 9.2x \\ 
%     \hline 
%    \end{tabular}    
%    }
%    \caption{Benchmark results: {\tt{VarPointsTo}} and {\tt{Throws}} is 
%    presented as tuples $(a,b)$, where $a$ is the total entries, $b$ is the average 
%    types being invoked on in {\tt{VarPointsTo}} case,
%     and average exception objects thrown in {\tt{Throws}} case. 
%     All times are in seconds.
%     $\infty$ denotes the analysis did not finish within 6000 seconds.}
%     \label{tbl:precision-result}
%\end{table} 


% % % current results, I will consider to add time. too.


